Improving the Explainability of Neural Sentiment Classifiers via Data Augmentation

Sentiment analysis has been widely used by businesses for social media opinion mining, especially in the financial services industry, where customers' feedbacks are critical for companies. Recent progress of neural network models has achieved remarkable performance on sentiment classification, while the lack of classification interpretation may raise the trustworthy and many other issues in practice. In this work, we study the problem of improving the explainability of existing sentiment classifiers. We propose two data augmentation methods that create additional training examples to help improve model explainability: one method with a predefined sentiment word list as external knowledge and the other with adversarial examples. We test the proposed methods on both CNN and RNN classifiers with three benchmark sentiment datasets. The model explainability is assessed by both human evaluators and a simple automatic evaluation measurement. Experiments show the proposed data augmentation methods significantly improve the explainability of both neural classifiers.

==> classifiers.tex <==
\section{Neural Sentiment Classifiers}
\label{sec:background}

% \subsection{Sentiment Classifiers}
% \label{subsec:sentiment}



==> tables/tab-case.tex <==
\begin{table}
  \centering
  \begin{tabular}{lp{0.3\textwidth}}
    \toprule
    Orig. Example & This is one of Polanski 's \emph{best} films\\
    Keywords & best\\
    Aux. Example & This is one of Polanski 's films\\
    \bottomrule
  \end{tabular}
  \caption{Creating an auxiliary example from the training set. The auxiliary example is part of the original example with sentiment keywords (e.g., \emph{best}) removed.}
  \label{tab:case}
\end{table}

==> tables/tab-eval-explanation.tex <==
\begin{table*}
  \renewcommand\arraystretch{1.5}
  \centering
  \small
  \begin{tabular}{lp{0.5\textwidth}llll}
    \toprule
    & Example & Ground & CNN & Keywords & \\
    & Text &  Truth & Prediction & Indication & Coherence \\
    \midrule
    \multicolumn{6}{l}{\emph{Coherent cases}}\\
    1.& if you sometimes like to go to the movies to have \textbf{fun}, wasabi \textbf{is} a \textbf{good} place to start & Positive & Positive & Positive & $\surd$ \\
    2.& \textbf{unintentionally} hilarious, the direction \textbf{unfocused}, the performances as \textbf{wooden} & Negative & Negative & Negative & $\surd$ \\
    3.& if this movie \textbf{were} a book, it would be a page turner, you can't \textbf{wait} to see what \textbf{happens} next & Positive & Negative & None & $\surd$ \\
    4.& it's a \textbf{great} \textbf{deal} of \textbf{sizzle} and very little steak & Negative & Positive & None & $\surd$ \\
    5.& though everything might be \textbf{literate} and \textbf{smart}, it never took off and \textbf{always} seemed static & Negative & Positive & Positive & $\surd$ \\
    6.& but \textbf{he} \textbf{somehow} pulls it \textbf{off} & Positive & Negative & Negative & $\surd$ \\
    \multicolumn{6}{l}{\emph{Incoherent cases}}\\
    7.& a real movie, about real people, that gives us a rare glimpse \textbf{into} a \textbf{culture} \textbf{most} of us don't know & Positive & Positive & None & $\times$ \\
    8.& fuller would surely have called this \textbf{gutsy} and at times \textbf{exhilarating} movie a \textbf{great} yarn & Positive & Positive & Negative & $\times$ \\
    9.& nearly \textbf{surreal}, dabbling in french, this is no \textbf{simple} movie, and you'll be taking a \textbf{risk} if you choose to see it & Negative & Positive & Negative & $\times$ \\
    10.& if it's possible for a sequel to \textbf{outshine} the original, \textbf{then} sl2 does \textbf{just} that & Positive & Negative & Positive & $\times$ \\
    11.& \textbf{cliches} are as thick as the \textbf{cigarette} \textbf{smoke} & Negative & Negative & Positive & $\times$ \\
    12.& it's as \textbf{flat} as an open can of pop \textbf{left} \textbf{sitting} in the sun & Negative & Negative & None & $\times$ \\
    \bottomrule
  \end{tabular}
  \caption{Examples of the coherent and incoherent cases, where the grasped keywords are presented in bold in each text.}
  \label{tab:eval-explanation}
\end{table*}

